Persona is a Double-edged Sword: Mitigating the Negative Impact of Role-playing Prompts in Zero-shot Reasoning Tasks

Recent studies demonstrate that prompting a role-playing persona to an LLM improves reasoning capability. However, assigning an adequate persona is difficult since LLMs are extremely sensitive to assigned prompts; thus, inaccurately defined personas sometimes hinder LLMs and degrade their reasoning capabilities. In this paper, we first investigate the potential negative impact of injecting persona into language models. Furthermore, we propose a novel framework, Jekyll \& Hyde, which ensembles the outcomes of both role-playing and neutral prompts to enhance the robustness of reasoning ability. Specifically, Jekyll \& Hyde predicts an appropriate persona using an LLM when defining the role-playing prompt. Then, Jekyll \& Hyde collects two potential solutions from role-playing and neutral prompts and selects a better solution using the LLM evaluator. The experimental analysis demonstrates that role-playing prompts sometimes distract LLMs, degrading their reasoning abilities in 7 out of 12 datasets in llama3. Meanwhile, Jekyll \& Hyde improve reasoning capabilities by selecting better choices among the potential solutions on twelve widely-used natural language reasoning datasets. In addition, we reveal that assigning LLM-generated personas obtains more stable results than handcrafted personas.

==> fig_texts/algorithm.tex <==
\algrenewcommand\algorithmicindent{1.5em}%
\algrenewcommand\algorithmicrequire{\textbf{Input:}}
\algrenewcommand\algorithmicensure{\textbf{Output:}}
\begin{algorithm}[H]
 \caption{Jekyll and Hyde framework process}
\begin{algorithmic}[1]
\small 
\Require a dataset $d \in \mathcal{D}$; a language model $M$; prompts $\{p\}$
\Ensure Solution $\mathcal{S}_{final}$
\State $\mathcal{S} \gets$ false  \Comment{\scriptsize{Whether pruning is complete or not}}
\small
\For {epoch = $1,2,...,N$}
    \small
    \State $\mathcal{B} \gets $ split $\mathcal{D}_{train}$ into mini-batches of size $\beta$
    \For{each batch $b \in \mathcal{B}$}
        \State compute a batch loss $\mathcal{L}_{\mathcal{P}}(b)$
    \EndFor
    \If{$\mathcal{L}_{\mathcal{P}}$ is converged}
        \If{$\mathcal{S}$ is false}
            \small
            \State $\mathcal{S} \gets$ true
            % \State sample a small subset $\Tilde{\mathcal{D}}_{train}$ and $\Tilde{\mathcal{D}}_{eval}$
            \For{each layer $l \in \mathcal{P}$}
                \State compute skill relevance $A_{i}(h^{l})$
            \EndFor
            \State sort neuron indices by $A_{i}(h^{l})$
            \State get skill-irrelevant neuron set $\mathcal{M}$
            \State skill-localize $\mathcal{P}$ by pruning $\mathcal{M}$
        \Else
            \State \textbf{break}
        \EndIf
    \EndIf
\EndFor
\Return $\mathcal{P}$

\end{algorithmic}
\label{algorithm:1}
\vspace{-0.02cm}
\end{algorithm}


==> fig_texts/fig1.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=1.0\linewidth]{fig_files/fig1_refined.pdf}
% \vspace{-0.6cm}
\caption{The example contains an ambiguous context; thus, the correct answer is \textit{"can't answer"} since it is impossible to judge which group corresponds to the answer for a given negative question (e.g., \textit{"What group of people uses drugs?"}).
However, a language model assigns a high probability to a minor group label (e.g., \textit{"poor people"}).
Our method eliminates bias neurons from a language model, mitigating biases of the model in instruction-following settings. 
}
\label{fig:intro1}
% \vspace{-1.cm}
\end{figure}


==> fig_texts/fig2.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.95\linewidth]{fig_files/fig2.pdf}
\vspace{-.2cm}
\caption{\textbf{Performance gaps in understanding instructions.} We plot the accuracies of Flan-T5-base about ten synonymous instructions for BBQ-SES, BBQ-Age, MRPC and RTE datasets. For example, the accuracy between instructions differed by up to 5\% and 15\% for BBQ-SES and MRPC, respectively.
These results reveal that an instruction-following model shows biases in understanding instructions.
The utilized instructions are described in detail in Appendix~\ref{appendix:inst-template}.
}
\label{fig:intro2}
\vspace{-0.4cm}
\end{figure}


==> fig_texts/fig3.tex <==
\begin{figure}[H]
\centerline{\includegraphics[width=1.0\linewidth]{fig_files/fig3.pdf}}
% \vspace{-0.2cm}
\caption{\textbf{Bias mitigation results for varying numbers of bias neurons.} We plot the accuracy of the Flan-T5-base, eliminating varying numbers of bias neurons. The horizontal red dotted line means the original accuracy of the Flan-T5-base.}
\label{fig:pruning-rates}
%
\end{figure}

==> fig_texts/fig4.tex <==
\begin{figure}[H]
\centerline{\includegraphics[width=1.0\linewidth]{fig_files/fig4.pdf}}
% \vspace{-0.2cm}
\caption{\textbf{Bias mitigation results for varying numbers of data samples to compute bias attribution.}
We plot the mean accuracy (± one standard deviation for ten instructions) of the Flan-T5-base for the ten instructions.}
\label{fig:num-samples}
%
\end{figure}


==> fig_texts/fig5.tex <==
\begin{figure}[H]
\centerline{\includegraphics[width=1.0\linewidth]{fig_files/fig5.pdf}}
% \vspace{-0.2cm}
\caption{\textbf{Skill knowledge preservation experiments.} 
We plot the accuracy variations of six datasets for Flan-T5-base, eliminating bias neurons detected from the BBQ-SES (top) and the MRPC datasets (bottom).
CRISPR determines the number of bias neurons by measuring the accuracy of the original datasets (source), the BBQ-SES and the MRPC, respectively.
Then, the bias-mitigated models are evaluated in each target dataset.}
\label{fig:knowl-transfer}
%
\end{figure}

==> fig_texts/fig_compare_sc.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.9\linewidth]{fig_files/sc_compare_new.pdf}

\caption{\textbf{Performance comparison with equal LLM execution counts} We plot Jekyll \& Hyde and other methods under the condition of having approximately same number of LLM executions. The orange and blue horizontal line indicates the performance of Base, and the performance of Persona, respectively.}
\label{fig:compare_sc}
\vspace{-0.45cm}
\end{figure}

==> fig_texts/table2.tex <==
\begin{table}[]
\centering
\small
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{l}
\toprule
\textbf{Dataset}: AQuA \\
\midrule
\textbf{Question}: On a map, the length of the road from Town F to Town G is measured\\to be 20 inches. On this map, 1/4 inch represents an actual distance of 10 miles.\\ What is the actual distance, in miles, from Town F to Town G along this road?\\Answer Choices: (A) 800 (B) 720 (C) 960 (D) 1140 (E) 1160 \\
\midrule
\textbf{prompt that assigns persona hand-crafted by Human}: \\ You are a Math teacher \quad\textcolor{red}{\ding{55}} \\ 
\midrule
\textbf{prompt that assigns persona generated by LLM}:\\ You are a Cartographer \quad\textcolor{green!80!black}{\checkmark}\\
\bottomrule
\end{tabular}
}
\caption{An example of Zero-Shot, Zero-Shot-CoT, and Role-Play Prompting on Last Letter Concatenation.}
\label{table2}
\end{table}

==> fig_texts/table3.tex <==
\begin{table*}[t]
\centering
\scalebox{0.95}{
\begin{tabular}{lcccccc} 
\toprule
\multirow{2}{*}{Method} & \multicolumn{6}{c}{Arithmetic} \\ 
\cmidrule(r){2-7} & MultiArith & GSM8K & AddSub & AQuA & SingleEq & SVAMP \\ 
\midrule
Few-Shot-CoT & 97.7       & 76.9 & 93.9   & 59.4                          & 98.8     & 82.2                            \\ 
\midrule
Zero-Shot               & \textbf{97.3}       & 76.0                & 88.6   & 53.5                          & \textbf{98.2}     & 75.3                            \\ 
Zero-Shot-CoT               & 95.0       & \textbf{79.6}                & 86.6   & 53.9                          & 96.9     & 76.3                            \\ 
Role-Play Prompting     & 97.0       & 78.2                & \textbf{91.1}   & \textbf{63.8}                          & 98.0     & \textbf{83.8}                            \\ 
\midrule
CoT in Zero-Shot &\checkmark  &\checkmark &\checkmark &\checkmark &\checkmark &\checkmark \\
\midrule
\multirow{2}{*}{Method} & \multicolumn{2}{c}{Common Sense} & \multicolumn{2}{c}{Symbolic Reasoning} & \multicolumn{2}{c}{Other  Tasks}  \\ 
\cmidrule(r){2-3}%
\cmidrule(r){4-5}%
\cmidrule(r){6-7}%

% \cline{2-7}
                        & CSQA       & Strategy            & Letter & Coin                          & Date     & Object                          \\ 
\midrule
Few-Shot-CoT               & 76.3       & 67.4                & 74.2   & 99.6                          & 78.9     & 56.7                            \\ 
\midrule
Zero-Shot               & 74.5       & 66.0                & 23.8   & 55.2                          & 67.8     & 38.7                            \\ 
Zero-Shot-CoT               & 68.8       & 65.8                & 53.2   & \textbf{98.8}                          & 65.9     & \textbf{73.5}                            \\
Role-Play Prompting     & \textbf{77.2}       & \textbf{67.0}                & \textbf{84.2}   & 89.4                          & \textbf{69.9}     & 67.7                            \\
\midrule
CoT in Zero-Shot &\checkmark  &\checkmark &\ding{55} &\ding{55} &\checkmark &\ding{55} \\
\bottomrule
\end{tabular}}
\caption{Accuracy comparison of Role-Play Prompting with Few-Shot-CoT,  Zero-Shot, Zero-Shot-CoT on each dataset. In the rows ``CoT in Zero-Shot", the check mark denotes that ChatGPT can spontaneously generate CoT on the corresponding dataset under the zero-shot setting, while the cross (wrong symbol) denotes otherwise.}
\label{tb: results}
\end{table*}

==> fig_texts/table5.tex <==
\begin{table}[H]
\centering
\resizebox{1.0\linewidth}{!}
{
\begin{tabular}{@{}ccccc@{}}
\toprule
Method & \hspace{0.5em}BBQ-SES\hspace{0.5em} & \hspace{0.5em}MRPC\hspace{0.5em} \\\bottomrule
CRISPR & 71.68 & 73.27 \\ %\midrule
(-) Max Token Agg & 71.32 & 72.19 \\
(-) Instance Weight Agg & 70.92 & 72.40 \\
(-) Skill Disentangle & 70.28 & 72.17  \\
Random & 65.62 & 61.15 \\ \bottomrule
\end{tabular}
}
\vspace{-0.1cm}
\caption{
\textbf{Ablation studies.} We report the accuracy of each method for BBQ-SES and MRPC datasets.
}
\label{table5}
\end{table}



==> fig_texts/table6.tex <==
\begin{table*}[h]
\centering
\resizebox{1.0\linewidth}{!}
{
\begin{tabular}{@{}ccl@{}}
\toprule
\hspace{0.5em} Dataset & Task & Instructions \\ \bottomrule

\rule{0in}{2.5ex}\multirow{10}{*}{BBQ datasets} & \multirow{10}{*}{Social bias QA} & For the subsequent context and question, decide on the most appropriate answer from the choices available.\\
& & Pick the best response among the answer options offered in relation to the given context and question.\\
& & Single out the exact answer from the choices below that best addresses the context and question.\\
& & Select the best answer among the below answers about the given context and question.\\
& & Given the context and question, identify the answer option that is most relevant from the choices available.\\
& & Choose the most appropriate response from the provided answer options in relation to the given situation and query.\\
& & For the subsequent scenario and query, choose the best answer among the following answer candidates.\\
& & Make your selection of the most appropriate answer from the given response options, considering the context and question at hand.\\
& & Decide on the most suitable response from the answer candidates provided, keeping the context and question in mind.\\
& & Choose the answer that aligns best with the provided scenario and question from the available response choices.\\ \midrule

\rule{0in}{2.5ex}\multirow{10}{*}{MRPC} & \multirow{10}{*}{Semantic textual matching} & Choose the best answer option for the equivalence of the following sentences. Are they equivalent or not equivalent?\\
& & Select the most fitting answer option to ascertain if the following sentences have the same meaning or not. Are they equivalent or not equivalent?\\
& & Choose the right answer option to see if the next sentences convey the same message or not. Are they equivalent or not equivalent?\\
& & Pick the correct answer option to establish if the given sentences are analogous in meaning or not. Are they equivalent or not equivalent?\\
& & Determine the right answer option to assess if the upcoming sentences share the same interpretation or differ. Are they equivalent or not equivalent?\\
& & For the subsequent sentences, select the most appropriate answer option. Are they equivalent or not equivalent?\\
& & Select the correct answer option to gauge if the mentioned sentences have congruent meanings or not. Are they equivalent or not equivalent?\\
& & Choose the fitting answer option to find out if the provided sentences resonate the same or differ. Are they equivalent or not equivalent?\\
& & Select the proper answer option for whether the ensuing sentences are of equivalent meaning or not. Are they equivalent or not equivalent?\\
& & Make a decision on the best answer option to clarify if the forthcoming sentences match in context or not. Are they equivalent or not equivalent?\\
\midrule

\rule{0in}{2.5ex}\multirow{10}{*}{RTE} & \multirow{10}{*}{Natural language inference} & Determine whether there is entailment between the given two sentences by selecting the most appropriate answer option. Are they entailment or not entailment?\\
& & Evaluate if there is an entailment relationship between the provided two sentences by choosing the most fitting answer option. Are they entailment or not entailment?\\
& & Assess if the presented two sentences demonstrate entailment by choosing the most suitable answer option. Are they entailment or not entailment?\\
& & Decide whether there is an entailment connection between the provided two sentences by selecting the most fitting answer option. Are they entailment or not entailment?\\
& & Evaluate if the given two sentences exhibit the relationship of entailment by choosing the most appropriate answer option. Are they entailment or not entailment?\\
& & Examine whether the two sentences provided indicate entailment by selecting the most suitable answer option. Are they entailment or not entailment?\\
& & Determine if there is an entailment relationship between the presented two sentences by choosing the most fitting answer option. Are they entailment or not entailment?\\
& & Ascertain whether the given two sentences display the relationship of entailment by selecting the most appropriate answer option. Are they entailment or not entailment?\\
& & Decide if there is entailment between the provided two sentences by choosing the most fitting answer option. Are they entailment or not entailment?\\
& & Determine whether the given two sentences show the relationship of entailment by selecting the most appropriate answer option. Are they entailment or not entailment?\\
\midrule

\rule{0in}{2.5ex}\multirow{10}{*}{QNLI} & \multirow{10}{*}{Natural language inference} & Determine whether there is entailment between the given question and sentence by selecting the most appropriate answer option. Are they entailment or not entailment?\\
& & Evaluate if there is an entailment relationship between the provided question and sentence by choosing the most fitting answer option. Are they entailment or not entailment?\\
& & Assess if the presented question and sentence demonstrate entailment by choosing the most suitable answer option. Are they entailment or not entailment?\\
& & Decide whether there is an entailment connection between the provided question and sentence by selecting the most fitting answer option. Are they entailment or not entailment?\\
& & Evaluate if the given question and sentence exhibit the relationship of entailment by choosing the most appropriate answer option. Are they entailment or not entailment?\\
& & Examine whether the question and sentence provided indicate entailment by selecting the most suitable answer option. Are they entailment or not entailment?\\
& & Determine if there is an entailment relationship between the presented question and sentence by choosing the most fitting answer option. Are they entailment or not entailment?\\
& & Ascertain whether the given question and sentence display the relationship of entailment by selecting the most appropriate answer option. Are they entailment or not entailment?\\
& & Decide if there is entailment between the provided question and sentence by choosing the most fitting answer option. Are they entailment or not entailment?\\
& & Determine whether the given question and sentence show the relationship of entailment by selecting the most appropriate answer option. Are they entailment or not entailment?\\
\bottomrule

\end{tabular}
}
\vspace{-0.1cm}
\caption{
\textbf{Instructions for each dataset.}
}
\vspace{-0.45cm}
\label{table6}
\end{table*}


==> fig_texts/table_case_study_addtional.tex <==
\begin{table*}[t]
\resizebox{1.0\textwidth}{!}
{
\centering
\begin{tabular}{cp{9cm}p{16cm}ccc}
\toprule
\hspace{0.5em}Dataset & Question ($q$) & Prediction of Solvers & \makecell{Evaluator$[q, r_1, r_2]$ \\ result} & \makecell{Evaluator$[q, r_2, r_1]$ \\ result} & \makecell{Final \\ prediction} \\ \bottomrule

\multirow{3}{*}{AQuA} & Two ants are standing side-by-side. One ant, which is 4 inches tall, casts a shadow that is 10 inches long. The other ant is 6 inches tall. Compute, in inches, the length of the shadow that the taller ant casts. \newline \textbf{Answer Choices:} (A) 36 (B) 28 (C) 42 (D) 15 (E) 20 & \textbf{Neutral Solver ($r_1$)} \newline \textbf{explanation:} A classic problem! Let\'s use the concept of similar triangles to solve this. We can draw a diagram: In this diagram, the ratio of the height of the ant to the length of its shadow is the same for both ants. Let\'s call this ratio "k", $ \cdots$. we can multiply the height by the ratio k to get: Shadow length = 6 × (2/5) = 12 inches So, the correct answer is: (C) 42. Therefore, among A through E, the answer is C \newline \textbf{persona: } None \newline \textbf{answer:} C \newline \newline
\textbf{Persona Solver($r_2$)} \newline \textbf{explanation:} A classic problem! Let's use the concept of similar triangles to solve this. We can draw a diagram: In this diagram, the ratio of the height of the ant to the length of its shadow is the same for both ants. $\cdots$. The correct answer is (D) 15. Therefore, among A through E, the answer is D \newline \textbf{persona: } Mathematician \newline \textbf{answer:} D
& \textbf{verdict:} $r_2$ & \textbf{verdict:} $r_2$ & D \\
\midrule

\multirow{3}{*}{AQuA} & Two ants are standing side-by-side. One ant, which is 4 inches tall, casts a shadow that is 10 inches long. The other ant is 6 inches tall. Compute, in inches, the length of the shadow that the taller ant casts. \newline \textbf{Answer Choices:} (A) 36 (B) 28 (C) 42 (D) 15 (E) 20 & \textbf{Neutral Solver ($r_1$)} \newline \textbf{explanation:} A classic problem! Let\'s use the concept of similar triangles to solve this. We can draw a diagram: In this diagram, the ratio of the height of the ant to the length of its shadow is the same for both ants. Let\'s call this ratio "k", $ \cdots$. we can multiply the height by the ratio k to get: Shadow length = 6 × (2/5) = 12 inches So, the correct answer is: (C) 42. Therefore, among A through E, the answer is C \newline \textbf{persona: } None \newline \textbf{answer:} C \newline \newline
\textbf{Persona Solver($r_2$)} \newline \textbf{explanation:} A classic problem! Let's use the concept of similar triangles to solve this. We can draw a diagram: In this diagram, the ratio of the height of the ant to the length of its shadow is the same for both ants. $\cdots$. The correct answer is (D) 15. Therefore, among A through E, the answer is D \newline \textbf{persona: } Mathematician \newline \textbf{answer:} D
& \textbf{verdict:} $r_2$ & \textbf{verdict:} $r_2$ & D \\
\midrule


\multirow{3}{*}{AQuA} & Two ants are standing side-by-side. One ant, which is 4 inches tall, casts a shadow that is 10 inches long. The other ant is 6 inches tall. Compute, in inches, the length of the shadow that the taller ant casts. \newline \textbf{Answer Choices:} (A) 36 (B) 28 (C) 42 (D) 15 (E) 20 & \textbf{Neutral Solver ($r_1$)} \newline \textbf{explanation:} A classic problem! Let\'s use the concept of similar triangles to solve this. We can draw a diagram: In this diagram, the ratio of the height of the ant to the length of its shadow is the same for both ants. Let\'s call this ratio "k", $ \cdots$. we can multiply the height by the ratio k to get: Shadow length = 6 × (2/5) = 12 inches So, the correct answer is: (C) 42. Therefore, among A through E, the answer is C \newline \textbf{persona: } None \newline \textbf{answer:} C \newline \newline
\textbf{Persona Solver($r_2$)} \newline \textbf{explanation:} A classic problem! Let's use the concept of similar triangles to solve this. We can draw a diagram: In this diagram, the ratio of the height of the ant to the length of its shadow is the same for both ants. $\cdots$. The correct answer is (D) 15. Therefore, among A through E, the answer is D \newline \textbf{persona: } Mathematician \newline \textbf{answer:} D
& \textbf{verdict:} $r_2$ & \textbf{verdict:} $r_2$ & D \\



\bottomrule
\end{tabular}
}
% \vspace{-0.1cm}
\caption{
\textbf{Qualitative analysis.} We conduct a qualitative analysis of Jekyll and Hyde on three datasets. Jekyll and Hyde's Persona Solver attains dynamic persona based on the Persona Generator (e.g., Classical Mythology Scholar). Additionally, examples reveal that Evaluator is working properly via selecting the correct answer among different solutions from each Solver.
}
% \vspace{-0.45cm}
\label{table:qualitative_analysis}
\end{table*}

==> fig_texts/table_case_study_full.tex <==
\begin{table*}[h]
\resizebox{1.0\linewidth}{!}
{
\centering
\begin{tabular}{@{}cp{10cm}p{10cm}p{10cm}ccc@{}}
\toprule
\hspace{0.5em} Dataset & Question ($q$) & Neutral Solver($r_1$) & Persona Solver($r_2$) & \makecell{Evaluator$[q, r_1, r_2]$ \\ result} & \makecell{Evaluator$[q, r_2, r_1]$ \\ result} & \makecell{Final \\ prediction} \\ \bottomrule

\multirow{3}{*}{AQuA} & Two ants are standing side-by-side. One ant, which is 4 inches tall, casts a shadow that is 10 inches long. The other ant is 6 inches tall. Compute, in inches, the length of the shadow that the taller ant casts. \textbf{Answer Choices:} (A) 36 (B) 28 (C) 42 (D) 15 (E) 20 & \textbf{explanation:} A classic problem! Let\'s use the concept of similar triangles to solve this. We can draw a diagram: In this diagram, the ratio of the height of the ant to the length of its shadow is the same for both ants. Let\'s call this ratio "k". For the first ant, we know that the height is 4 inches and the shadow is 10 inches, so we can write: k = 4/10 = 2/5 Now, we can use this ratio to find the length of the shadow of the taller ant. Since the height of the taller ant is 6 inches, we can multiply the height by the ratio k to get: Shadow length = 6 × (2/5) = 12 inches So, the correct answer is: (C) 42 Therefore, among A through E, the answer is C  & \textbf{explanation:} A classic problem! Let's use the concept of similar triangles to solve this. We can draw a diagram: In this diagram, the ratio of the height of the ant to the length of its shadow is the same for both ants. We can write this as: 4/10 = 6/x. To solve for x, we can cross-multiply: 4x = 60 \n Divide both sides by 4: x = 15. So, the taller ant casts a shadow that is 15 inches long. The correct answer is (D) 15. Therefore, among A through E, the answer is D & \textbf{verdict:} $r_2$ & \textbf{verdict:} $r_2$ & D \\
&  & \textbf{persona: } None & \textbf{persona: } Mathematician & & & \\
&  & \textbf{answer:} C & \textbf{answer:} D & & & \\

\midrule

% \multirow{3}{*}{Singleeq} & \multirow{3}{*}{?} & \textbf{persona:} None & \textbf{persona:} & \textbf{explanation:} & \textbf{explanation:} & ? \\
% & & \textbf{explanation:} None & \textbf{explanation:} & \textbf{verdict:} & \textbf{verdict:} & \\
% & & \textbf{explanation:} None & \textbf{explanation:} & \textbf{verdict:} & \textbf{verdict:} & \\

% \midrule

\multirow{3}{*}{Strategy} & Is Saturn named after king of gods in Greek mythology? & \textbf{explanation:} Yes, the planet Saturn is indeed named after the Roman god Saturnus, who was the equivalent of the Greek god Cronus. In Roman mythology, Saturnus was the god of agriculture, fertility, and time, and was often depicted as a wise and just ruler. The planet Saturn was discovered in 1610 by Galileo Galilei, and it was initially known as "Jove\'s Scourge" or "the Seventh Planet" (since it was the seventh planet from the Sun to be discovered). However, in 1847, the German astronomer Johann Elert Bode suggested that the planet be named after the Roman god Saturnus, as a nod to the Roman mythology and the planet\'s ring system, which resembles the god\'s crown. So, while the planet Saturn is not directly named after the Greek god Cronus, it is indeed named after the Roman god Saturnus, who shares a similar mythological background and symbolism with Cronus. Therefore, the answer (Yes or No) is yes  & \textbf{explanation:} A great question! However, I must correct you - Saturn is actually named after the Roman god Saturnus, not the Greek god of the gods, Zeus. In Roman mythology, Saturnus was the god of agriculture, fertility, and time. He was often depicted as a wise and just ruler, and his name is derived from the Latin word "sater," meaning "sower" or "planter." The planet Saturn, which was discovered in 1610 by Galileo Galilei, was named after the Roman god because of its slow orbital period, which was thought to be reminiscent of Saturnus\'s association with time and the cycles of nature. In Greek mythology, the equivalent of Saturnus is Cronus, who was the Titan god of agriculture and time. Cronus was known for castrating his father Uranus and taking over the throne of the gods. However, the planet Saturn was not named after Cronus, but rather after the Roman god Saturnus. Therefore, the answer (Yes or No) is no & \textbf{verdict:} $r_2$ & \textbf{verdict:} $r_2$ & no \\
&  & \textbf{persona: } None & \textbf{persona: } Classical Mythology Scholar & & & \\
&  & \textbf{answer:} yes & \textbf{answer:} no & & & \\

% \midrule

% \multirow{3}{*}{Letters} & \multirow{3}{*}{?} & \textbf{persona:} None & \textbf{persona:} & \textbf{explanation:} & \textbf{explanation:} & ? \\
% & & \textbf{explanation:} None & \textbf{explanation:} & \textbf{verdict:} & \textbf{verdict:} & \\
% & & \textbf{explanation:} None & \textbf{explanation:} & \textbf{verdict:} & \textbf{verdict:} & \\

\midrule

\multirow{3}{*}{Object} & Alice, Bob, and Claire are holding a white elephant gift exchange. At the start of the event, they are each holding a present of a different color: Alice has a orange ball, Bob has a purple present, and Claire has a blue present. As the event progresses, pairs of people swap gifts. First, Claire and Alice swap their gifts. Then, Alice and Bob swap their gifts. Finally, Bob and Claire swap their gifts. At the end of the event, Alice has the Which choice is true ? \textbf{Answer Choices:} (A) orange ball. (B) purple present. (C) blue present. & \textbf{explanation:} Let's follow the gift-swapping process: 1. Claire and Alice swap gifts: Claire gets the orange ball, and Alice gets the blue present. 2. Alice and Bob swap gifts: Alice gets the purple present, and Bob gets the blue present. 3. Bob and Claire swap gifts: Bob gets the blue present (which he already had), and Claire gets the purple present. At the end of the event, Alice has the purple present. Therefore, the correct answer is: (B) purple present. Therefore, among A through C, the answer is B  & \textbf{explanation:} A fun gift exchange problem! Let's break it down step by step: 1. Claire and Alice swap gifts: Claire gets the orange ball, and Alice gets the blue present. 2. Alice and Bob swap gifts: Alice gets the purple present, and Bob gets the blue present. 3. Bob and Claire swap gifts: Bob gets the blue present back (which he got from Alice), and Claire gets the purple present. Now, let's see who has which gift at the end: * Alice has the purple present (from Bob) and the blue present (from Claire). * Bob has the blue present (from Claire) and the orange ball (from Claire and Alice). * Claire has the orange ball (from Alice) and the purple present (from Bob). So, the correct answer is: (A) orange ball. Therefore, among A through C, the answer is A & \textbf{verdict:} $r_1$ & \textbf{verdict:} $r_1$ & B \\
&  & \textbf{persona: } None & \textbf{persona: } Gift Exchange Analyst & & & \\
&  & \textbf{answer:} B & \textbf{answer:} A & & & \\
\bottomrule
\end{tabular}
}
% \vspace{-0.1cm}
\caption{
\textbf{Qualitative analysis.} We conduct a qualitative analysis of Jekyll \& Hyde on three datasets. Jekyll \& Hyde's Persona Solver attains dynamic persona based on the Persona Generator (e.g. Classical Mythology Scholar). Additionally, examples reveal that Evaluator is working properly via selecting the correct answer among different solutions from each Solver.
}
% \vspace{-0.45cm}
\label{table:qualitative_analysis}
\end{table*}

% \begin{table*}[h]
% \resizebox{1.0\linewidth}{!}
% {
% \centering
% \begin{tabular}{@{}ccp{15cm}@{}}
% \toprule
% \hspace{0.5em} Dataset & & \\ 
% \bottomrule
% \multirow{6}{*}{AQuA} & question & Two ants are standing side-by-side. One ant, which is 4 inches tall, casts a shadow that is 10 inches long. The other ant is 6 inches tall. Compute, in inches, the length of the shadow that the taller ant casts. \textbf{Answer Choices:} (A) 36 (B) 28 (C) 42 (D) 15 (E) 20 \\
% \cmidrule{2-3}
% & base LLM output $r_1$ & \textbf{explanation:} A classic problem! Let\'s use the concept of similar triangles to solve this. We can draw a diagram: In this diagram, the ratio of the height of the ant to the length of its shadow is the same for both ants. Let\'s call this ratio "k". For the first ant, we know that the height is 4 inches and the shadow is 10 inches, so we can write: k = 4/10 = 2/5 Now, we can use this ratio to find the length of the shadow of the taller ant. Since the height of the taller ant is 6 inches, we can multiply the height by the ratio k to get: Shadow length = 6 × (2/5) = 12 inches So, the correct answer is: (C) 42 Therefore, among A through E, the answer is C \\
% & & persona: None \\
% & & answer: \\
% \cmidrule{2-3}
% & persona LLM output $r_2$ & \textbf{explanation:} A classic problem! Let's use the concept of similar triangles to solve this. We can draw a diagram: In this diagram, the ratio of the height of the ant to the length of its shadow is the same for both ants. We can write this as: 4/10 = 6/x. To solve for x, we can cross-multiply: 4x = 60 \n Divide both sides by 4: x = 15. So, the taller ant casts a shadow that is 15 inches long. The correct answer is (D) 15. Therefore, among A through E, the answer is D \\
% & & persona: Mathematician \\
% & & answer: \\
% \cmidrule{2-3}
% & \makecell{Evaluator$[q, r_1, r_2]$ \\ result} & \\
% \cmidrule{2-3}
% & \makecell{Evaluator$[q, r_2, r_1]$ \\ result} & \\
% \cmidrule{2-3}
% & \makecell{Final \\ prediction} & D
% \bottomrule
% \end{tabular}}
% % \vspace{-0.1cm}
% \caption{Sample
% }
% % \vspace{-0.45cm}
% \label{table:qualitative_analysis}
% \end{table*}


==> fig_texts/table_confusion_matrix-coinflip.tex <==
% \begin{table}[]
% \centering
% \small
% \begin{tabular}{c|c|c|c|c}

% \toprule
% Method&\multicolumn{4}{c}{\makecell{Persona Solver \\ (w/ Persona)}} \\
% \midrule
% \multirow{5}{*}{\makecell{Neutral Solver \\ (w/o Persona)}} & AQuA & Wrong & Right & Total \\
% \cmidrule{2-5}
% % \midrule
% & Wrong & 33.07\% & 15.75\% & 48.82\% \\
% \cmidrule{2-5}
% &Right& \textcolor{red}{\textbf{13.78\%}} & 37.40\% & 51.18\%\\
% \cmidrule{2-5}
% & Total & 46.85\% & 53.15\% & 100\% \\
% \bottomrule
% \end{tabular}
% \caption{\textbf{Confusion matrix between Neutral Solver (w/o Persona) and its Persona Solver (w/ Persona) on AQuA dataset.} we compute each model’s correctness, exhibiting the result in a confusion matrix form. Neutral Solver and Persona Solver means an LLM without persona and an LLM with persona, respectively.}
% \vspace{-15pt}
% \label{table: confusion matrix aqua}
% \end{table}

\begin{table}[]
\centering
\small
% \resizebox{1.0\linewidth}{!}{
\begin{tabular}{c|c|c|c}

\toprule
Method&\multicolumn{3}{c}{\makecell{Persona Solver \\ (w/ Persona)}} \\
\midrule
\multirow{5}{*}{\makecell{Neutral Solver \\ (w/o Persona)}} & Coin Flip & Wrong & Right \\
\cmidrule{2-4}
% \midrule
& Wrong & 4.60\% & 4.00\% \\
\cmidrule{2-4}
&Right& \textcolor{red}{\textbf{18.00\%}} & 73.40\%\\
\bottomrule
\end{tabular}
% }
\caption{Confusion matrix between Neutral Solver (w/o Persona) and its Persona Solver (w/ Persona) on Coin Flip dataset.}
\vspace{-15pt}
\label{table: confusion matrix coinflip}
\end{table}

==> fig_texts/table_confusion_matrix-objectTracking.tex <==
% \begin{table}[]
% \centering
% \small
% \begin{tabular}{c|c|c|c|c}

% \toprule
% Method&\multicolumn{4}{c}{\makecell{Persona Solver \\ (w/ Persona)}} \\
% \midrule
% \multirow{5}{*}{\makecell{Neutral Solver \\ (w/o Persona)}} & AQuA & Wrong & Right & Total \\
% \cmidrule{2-5}
% % \midrule
% & Wrong & 33.07\% & 15.75\% & 48.82\% \\
% \cmidrule{2-5}
% &Right& \textcolor{red}{\textbf{13.78\%}} & 37.40\% & 51.18\%\\
% \cmidrule{2-5}
% & Total & 46.85\% & 53.15\% & 100\% \\
% \bottomrule
% \end{tabular}
% \caption{\textbf{Confusion matrix between Neutral Solver (w/o Persona) and its Persona Solver (w/ Persona) on AQuA dataset.} we compute each model’s correctness, exhibiting the result in a confusion matrix form. Neutral Solver and Persona Solver means an LLM without persona and an LLM with persona, respectively.}
% \vspace{-15pt}
% \label{table: confusion matrix aqua}
% \end{table}

\begin{table}[]
\centering
\small
% \resizebox{1.0\linewidth}{!}{
\begin{tabular}{c|c|c|c}

\toprule
Method&\multicolumn{3}{c}{\makecell{Persona Solver \\ (w/ Persona)}} \\
\midrule
\multirow{5}{*}{\makecell{Neutral Solver \\ (w/o Persona)}} & Object Tracking & Wrong & Right \\
\cmidrule{2-4}
% \midrule
& Wrong & 46.67\% & 18.13\% \\
\cmidrule{2-4}
&Right& \textcolor{red}{\textbf{12.93\%}} & 22.27\%\\
\bottomrule
\end{tabular}
% }
\caption{Confusion matrix between Neutral Solver (w/o Persona) and its Persona Solver (w/ Persona) on Object Tracking dataset.}
\vspace{-15pt}
\label{table: confusion matrix object tracking}
\end{table}

==> fig_texts/table_confusion_matrix-strategyqa.tex <==
% \begin{table}[]
% \centering
% \small
% \begin{tabular}{c|c|c|c|c}

% \toprule
% Method&\multicolumn{4}{c}{\makecell{Persona Solver \\ (w/ Persona)}} \\
% \midrule
% \multirow{5}{*}{\makecell{Neutral Solver \\ (w/o Persona)}} & AQuA & Wrong & Right & Total \\
% \cmidrule{2-5}
% % \midrule
% & Wrong & 33.07\% & 15.75\% & 48.82\% \\
% \cmidrule{2-5}
% &Right& \textcolor{red}{\textbf{13.78\%}} & 37.40\% & 51.18\%\\
% \cmidrule{2-5}
% & Total & 46.85\% & 53.15\% & 100\% \\
% \bottomrule
% \end{tabular}
% \caption{\textbf{Confusion matrix between Neutral Solver (w/o Persona) and its Persona Solver (w/ Persona) on AQuA dataset.} we compute each model’s correctness, exhibiting the result in a confusion matrix form. Neutral Solver and Persona Solver means an LLM without persona and an LLM with persona, respectively.}
% \vspace{-15pt}
% \label{table: confusion matrix aqua}
% \end{table}

\begin{table}[]
\centering
\small
% \resizebox{1.0\linewidth}{!}{
\begin{tabular}{c|c|c|c}

\toprule
Method&\multicolumn{3}{c}{\makecell{Persona Solver \\ (w/ Persona)}} \\
\midrule
\multirow{5}{*}{\makecell{Neutral Solver \\ (w/o Persona)}} & StrategyQA & Wrong & Right \\
\cmidrule{2-4}
% \midrule
& Wrong & 19.39\% & 12.31\% \\
\cmidrule{2-4}
&Right& \textcolor{red}{\textbf{10.31\%}} & 57.99\%\\
\bottomrule
\end{tabular}
% }
\caption{Confusion matrix between Neutral Solver (w/o Persona) and its Persona Solver (w/ Persona) on StrategyQA dataset.}
\vspace{-15pt}
\label{table: confusion matrix strategyqa}
\end{table}

==> fig_texts/table_effect_on_fixed_persona.tex <==
\begin{table}[]
\centering
\small
\scalebox{0.7}{
\begin{tabular}{ccccccc}
\toprule
\multirow{2}{*}{Method} & & \multicolumn{4}{c}{Datasets} & \multirow{2}{*}{Average} \\
& & MultiArith & SingleEq & date & coin & \\
\midrule
\multirow{4}{*}{\makecell{LLM \\ generated persona}} & trial 1 & 590 & 486 & 295 & 492 & \\
& trial 2 & 590 & 482 & 293 & 492 & \\
& trial 3 & 589 & 483 & 288 & 490 & \\
& Average & 589.67 & \textbf{483.67} & \textbf{292} & \textbf{491.33} & \textbf{464.17} \\
& stdev & 0.577 & 2.081 & 3.605 & 1.154 & \textbf{1.854} \\
% \cmidrule{2-7}
\midrule
% &Wrong & 33.07\% & 15.75\% & 48.82\% \\
\multirow{4}{*}{\makecell{handcrafted \\ persona}} & trial 1 & 592 & 481 & 293 & 489 & \\
& trial 2 & 590 & 477 & 286 & 487 & \\
& trial 3 & 592 & 483 & 294 & 486 & \\
& Average & \textbf{591.33} & 480.33 & 291 & 487.33 & 462.5 \\
& stdev & 1.154 & 3.055 & 4.358 & 1.527 & 2.524 \\
\bottomrule
\end{tabular}}
\caption{\textbf{performance using handcrafted persona LLM and LLM generated persona LLM for Jekyll and Hyde} Result shows that most of datasets presents better averaged performance when using LLM generated persona. In addition, utilizing LLM-generated persona influence the framework to have lower standard deviation comparing to handcrafted persona, thereby showing better stability in practice.} 
\vspace{-15pt}
\label{table:Effects of persona}
\end{table}

==> fig_texts/table_main_result.tex <==
\begin{table*}[h]
\centering
\resizebox{1.0\linewidth}{!}
{
\begin{tabular}{@{}cccccccccccccc@{}}
\toprule
\hspace{0.5em} Models & Method & Multiarith & GSM8K & AddSub & AQuA & SingleEq & SVAMP & CSQA & Strategy & Letter & Coin & Date & Object \\ 
% & CoT in Zero-shot & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \quad{\ding{55}} & \quad{\ding{55}} & \checkmark & \quad{\ding{55}} \\
\bottomrule

\rule{0in}{2.5ex}\multirow{4}{*}{\makecell{GPT-4 \\ (220B*8)}} & Base & \textbf{98.33\%} & 92.95\% & 97.22\% & 67.32\% & 98.62\% & 91.80\% & 80.10\% & 76.03\% & 18.80\% & 65.60\% & 78.59\% & 45.60\% \\
& Persona & 97.67\% & 93.86\% & 97.47\% & 75.59\% & 98.43\% & 90.80\% & 80.75\% & 76.29\% & 92.60\% & 72.40\% & 77.51\% & 58.67\% \\
% & CoT & 97.83\% & 0.00\% & 97.22\% & 74.41\% & 98.43\% & 91.20\% & 0.00\% & 0.00\% & 86.60\% & 74.00\% & 79.95\% & 61.20\% \\
\cmidrule{2-14}
& Jekyll \& Hyde & 98.00\% & \textbf{95.30\%} & \textbf{97.72\%} & \textbf{77.56\%} & \textbf{99.02\%} & \textbf{92.60\%} & \textbf{81.33\%} & \textbf{77.16\%} & \textbf{93.00\%} & \textbf{79.80\%} & \textbf{81.57\%} & \textbf{61.60\%} \\
\midrule

\rule{0in}{2.5ex}\multirow{4}{*}{\makecell{GPT-3.5-turbo \\ (20B)}} & Base & 97.00\% & 80.97\% &	88.10\% &	56.30\% &	97.24\% &	74.50\% &	77.07\% &	67.38\% &	24.60\% &	54.60\% &	68.02\% &	36.67\% \\
& Persona & 97.33\% &	83.70\% &	92.91\% &	57.87\% &	97.44\% &	82.30\% &	75.76\% &	67.42\% &	49.00\% &	58.40\% &	72.09\% &	46.27\% \\
% & CoT & 97.67\% &	 &	89.37\% &	62.60\% &	97.64\% & &	& & 46.40\% &	57.60\% &	\textbf{75.61\%} &	41.33\% \\
\cmidrule{2-14}
& Jekyll \& Hyde & \textbf{98.50\%} &	\textbf{85.14\%} &	\textbf{93.16\%} &	\textbf{64.17\%} &	\textbf{98.23\%} &	\textbf{83.00\%} & \textbf{77.23\%} & \textbf{67.90\%} &	\textbf{53.20\%} &	\textbf{59.60\%} &	\textbf{72.63\%} &	\textbf{46.67\%} & \midrule

\rule{0in}{2.5ex}\multirow{4}{*}{\makecell{llama3 \\ (8B)}} & Base & 98.33\% & 76.50\% & 88.35\% & 47.24\% & 93.70\% & 83.20\% & 73.14\% & 68.30\% & 86.40\% & 95.40\% & 77.51\% & 44.93\% \\
& Persona & 97.33\% & 78.77\% & 88.35\% & 53.15\% & 91.14\% & 84.70\% & 72.15\% & 70.31\% & 86.00\% & 95.00\% & 74.80\% & 49.07\% \\
% & CoT & \textcolor{red}{\textbf{0.67 (-0.77)}} & \textcolor{red!60}{\textbf{0.90 (-0.28)}} & \textcolor{red}{\textbf{0.69 (-0.62)}} & \textcolor{red}{\textbf{0.65 (-3.52)}} & \textcolor{red}{\textbf{0.66 (-2.00)}} & \textcolor{red}{\textbf{0.51 (-1.22)}} \\
\cmidrule{2-14}
& Jekyll \& Hyde & \textbf{98.33\%} & \textbf{81.12\%} & \textbf{91.14\%} & \textbf{53.54\%} & \textbf{95.67\%} & \textbf{86.80\%} & \textbf{74.12\%} & 69.91\% & \textbf{86.80\%} & \textbf{98.40\%} & \textbf{79.95\%} & \textbf{49.47\%} \\
\bottomrule
\end{tabular}
}
% \vspace{-0.1cm}
\caption{
\textbf{Main results.} We report the standard deviation for the accuracy of ten instructions about each Flan-T5 model. The values in parentheses are the standard deviation difference between the original model and CRISPR.
CRISPR alleviates the understanding gap between synonymous instructions, increasing the performance of each instruction. 
Red-colored values mean that the understanding gap is alleviated.
}
% \vspace{-0.45cm}
\label{table:main_result}
\end{table*}

==> fig_texts/wherebias.tex <==
\begin{figure}[H]
\centerline{\includegraphics[width=1.\linewidth]{fig_files/wherebias.pdf}}
\vspace{-0.2cm}
\caption{\textbf{Where do biases come from?}}
\label{where-bias}
%
\end{figure}

==> texts/experiments_old.tex <==
\subsection{Experimental setup}
\paragraph{Datasets.}
We conduct our experiments across 12 datasets used in prior research \cite{kong2024better, kojima2022large} categorized in 4 categories: (1) arithmetic, including MultiArith\cite{multiarith}, GSM8K\cite{gsm8k}, AddSub\cite{addsub}, AQUA-RAT\cite{aqua}, SingleEq\cite{singleeq}, and SVAMP\cite{svamp} (2) commonsense reasoning, including CSQA\cite{csqa} and StrategyQA\cite{strategy} (3) symbolic reasoning, including Last Letter Concatenation and Coin Flip\cite{chain} (4) other, including Date Understanding and Tracking Shuffled Objects from BIG-bench \cite{srivastava2022beyond} More details can be found in Appendix.

\paragraph{Models.}
We utilize two black box large language model released from Openai, which are GPT-4\cite{openai2023gpt4}, and GPT-3.5-turbo, and one open source large language model llama3\cite{llama3modelcard}. These models are used as a backbone of our Framework.

\paragraph{Implementation details.}
To evaluate Jekyll and Hyde (J\&H), we utilized 12 datasets and set handcrafted persona for each dataset. Details about the persona for each dataset can be found in the Appendix. We evaluate three case for each dataset, (1) base model which is a LLM without persona (2) expert persona LLM, a LLM with persona generated by LLM for every instance of the dataset, and (3) Jekyll and Hyde, our proposed Framework. Specifically, we investigate the model's performance by computing an exact match with the provided label of each dataset. When using the LLM as an evaluator in Jekyll and Hyde, we set the max attempt $k$ to 5 and temperature $\tau$ to $0.7$. The details for determining the hyperparameters are shown in section \ref{section:hyperparameters}. In the perspective of mitigating position bias, we compared our Framework with MEC + BPC\cite{wang2023large}, following their original implementation, including the hyper-parameter setting. In order to provide robust results, we executed each model three times and averaged their performance, including standard deviation. A more detailed configuration of Jekyll and Hyde(J\&H) and other baselines can be found in Appendix ??.

\input{fig_texts/table:main_result_new}

\subsection{Better performance using Jekyll \& Hyde}
 Table \ref{table:main_result} exhibits the performance of different methods on twelve different datasets in the metric of accuracy. The result possesses several points. 1) Persona does not improve the model unconditionally. According to the result, several datasets show that performance is better in using LLM without persona rather than persona-assigned LLM. Specifically, blah blah blah. 2) Using Jekyll and Hyde framework improves the model performance. By leveraging the evaluator, performance has increased in most of the datasets regardless of the model type. In detail, blah blah blah. 3) The performance gap between (1) Base and using (4) Jekyll and Hyde gets larger proportional to the size of the backbone model. This happens due to the effect of persona assigned LLM,

 
 \input{fig_texts/table:main_result_new2}

\subsection{Ablation of setting number of max attempts $k$ and Temperature $\tau$}
 When using Jekyll and Hyde, LLM designated as an evaluator requires some hyperparameters, which are the number of max attempts $k$, and temperature of LLM $\tau$. We conduct a experiment for each hyperparameter to examine the impact of them effecting the performance of the Framework. For the number of max attempts of evaluator, we compared four different values of $k$, namely 1,2,5, and 10 by computing the Framework's performance. As shown in figure ??, we compared the performance executed from llama3-8b-8192 as a backbone model, and found out performance of the Framework increases as the number of attempts increases. Despite of the improvement of the Framework, increasing the number of attempts leads to high cost burden of the Framework. Since the enhancement of the Framework based on their cost is getting smaller as the number of the max attempt increase, we decided to use 5 as our default setting, which can balance the performance of the Framework and prevent fining the model excessively.

 \input{fig_texts/fig:hyperparameter_setting}

 We further investigate the impact of LLM's temperature by comparing the performance of the Framework. We utilized four different temperatures for our experiment, which are 0.1, 0.4, 0.7, and 1.0. Figure ?? shows that temperature 0.7 exhibits the optimal performance among others. We believe that having a low temperature will generate the same answer from the model repetitively, ending up getting incorrect from the model frequently. Utilizing a high temperature for the evaluator, might generate inconsistent answers which hinders from generating a consistent answer from both evaluators. Thus, we leverage $0.7$ as our temperature for the evaluator by default.

\label{section:hyperparameters}

\subsection{Effects of using LLM generated persona}

 Illustrated in section \ref{section:persona_selection}, we choose to use LLM generated persona rather than utilizing handcrafted persona for our paper. While LLM generated persona has better flexibility than handcrafted persona since handcrafted persona requires human work for designating a specific persona for a particular dataset, it is unclear whether LLM generated persona yields better performance than handcrafted persona. We conduct an experiment that checks the impact of assigning persona to an LLM for each method. For the experiment, we use two datasets, namely aqua, and object tracking. Using LLama3-8b model as a backbone model, we run the model three times for each dataset and compute the average performance, and standard deviation for each dataset to verify the robustness of the method. In addition, we utilize three different human handcrafted persona for each run in order to check the robustness of the performance. Specifically, three handcrafted persona for aqua dataset are 1) Math teacher, 2) Mathematician, and 3) Math Tutor. For Object tracking, 1) Observer, 2) Recorder, 3) Logical Reasoner is leveraged. As shown in table \ref{table:variance_of_persona}, we found that 1) the average performance shows that no one method dominates the other, instead each method could be effective depending on the dataset; 2) the value of standard deviation shows that using LLM-generated persona derives smaller standard deviation than using handcrafted persona. This implies that performance could vary depending on the designated persona when using a handcrafted persona. Therefore, we could consider that using LLM-generated persona stabilizes the model to have consistent results regardless of persona changes in each instance.

\input{fig_texts/table:variance_of_persona}

\subsection{Does persona generated from different LLM affects the LLM solver's performance?}
\label{section:same_llm_better_performance}

Due to the impact of role playing prompting towards LLMs, assigning persona enhance the reasoning capability of LLM. In Jekyll \& Hyde, we adopted a process that generates an appropriate persona for the given question by utilizing the LLM; however, it is unclear that using the same LLM for generating proper persona, and solving the question presents the optimal performance. We demystify the relationship between persona generator and persona solver by substituting the backbone model and computing the average accuracy for each dataset. To analysis the impact of using same backbone model, we used llama3-8b for the persona solver, and run three LLMs as our backbone model for the persona solver, involving llama3-8b, gpt-3.5-turbo, and gpt-4. Additionally, we utilized five different datasets, which are aqua, addsub, coin, date, and object. Results can be found in table \ref{table:effect_of_different_llm}. As is shown, we notice that using the same LLM as a backbone model reveals the optimal performance, while using different LLMs for persona generator. Specifically, 3 out of 5 datasets showed that using the same LLM leads to the optimal performance.

\input{fig_texts/table:same_llm_persona}


\subsection{Mitigating Position Bias}

% \paragraph{Detecting Position Bias} In order to improve Jekyll and Hyde, the performance of LLM as an evaluator is crucial, since selecting the correct answer among two solutions directly influence the framework performance. While we prompt the model with inserting solution from each LLM, previous studies claim that LLM suffers from positional bias when it comes to using LLM as an evaluator. Specifically, positional bias hinders LLM by selecting solution that priorly appears in the prompt, which is not related in selecting correct solution. To address the aforementioned bias, we quantified the impact of positional bias from the backbone model based on several datasets. In detail, we insert the solutions alternately, run the evaluator LLM for each prompt, and analyze the result from each evaluator by counting how many questions were affected by the order. As shown in table ??, the entire back bone model were affected by position bias. In addition, smaller models in respect of the size of the model are severely impacted by positional bias, thereby leading to low performance. In total, we demystified one of the issue that affects the Framework to have lower performance rate, and necessity of mitigating position bias inside evaluator LLM.

\paragraph{Mitigating Position Bias} To enhance the performance of the task, it is necessary to mitigate position bias from the LLM evaluator. For further analysis of the Framework's mitigation process, we compared the performance of Jekyll \& Hyde with the existing two position bias mitigation methods and Jekyll \& Hyde without position bias mitigation. We used 6 different datasets to test in general use case. Existing methods are implemented using the original setting from their original papers. Results can be found in table \ref{table:pos_bias}. According to the result, we find that 1) the evaluator within Jekyll \& Hyde derives the highest performance among the other methods from most datasets, regardless of the type of the backbone model; 2) Despite using the evaluator of Jekyll \& Hyde superficially looks like having a marginal impact on performance improvement, comparing with the oracle answer shows that Jekyll \& Hyde actually influence a huge impact on having idealistic performance to the model when considering the fact that oracle answer is the ideal performance when ensembling persona solver, and neutral solver.

\input{fig_texts/table:comparing_pos_bias}

\subsection{Qualitative analysis}
We qualitatively analyze our method on five different datasets, namely aqua, singleeq, strategyqa, last letter, and object tracking. Table \ref{table:qualitative_analysis} exhibits the result of qualitative analysis. These results reveal that the persona is dynamically generated based on the question from the LLM, stating different personas (i.g., Data analyst, physician) for different arithmetic questions. Additionally, running the evaluator by alternately inserting the solution of each LLM eventually gives a consistent verdict, which mostly ends up deriving the correct output for the given question. This meticulous process aids the framework in mitigating position bias that exists inside the LLM when using it as an evaluator, Increasing the performance of the framework.
\input{fig_texts/table:case_study}

==> texts/methods_old.tex <==
% Need to put figure about whole architecture here
 In this section, we demonstrate the process of Jekyll and Hyde (J\&H). Specifically, we select an appropriate persona based on the given question. Then, we execute both LLMs (LLM with persona, and LLM without persona) simultaneously. Finally, we insert two solutions from the previous step into the LLM designated as an evaluator, and receive a final answer based on the decision from the evaluator. We described the entire framework process in Algorithm \ref{algorithm:1}

\input{fig_texts/algorithm}

\subsection{Persona definement}

\label{section:persona_selection}
% first draft
%  We utilize two methodologies to designate a persona for the given question. For investigating better method between two methodologies, we format a system prompt and transform the prompt via assigning persona.The first method is using human hand-crafted persona based on the datasets. Formally, if the input $x$ is from the dataset $d \in \mathcal{D}$, then handcrafted persona $\mathcal{P}_{d, fixed}$ is returned from function $f$ as follows:
% \begin{equation}
% \begin{aligned}
%     \mathcal{P}_{d, fixed} = f(x, d) \:\:\:\:\: \\
%     \textbf{where}\ d \in \{d'|d' \in \mathcal{D}\}
% \end{aligned}
% \label{eq:handcrafted_persona_selection}
% \end{equation}
% \noindent Where handcrafted Persona $\mathcal{P}_d$ is available when the given input $x$ is included in one of the datasets in $\mathcal{D}$.

%  The second method is generating persona via LLM. By designing a prompt that could recommend a persona based on the given question, LLM could generate persona that are relevant to solve the problem. Suppose the given input is $x$, then the corresponding persona $\mathcal{P}_{expert}$ could be generated by the llm as defined below:
%  \begin{equation}
%  \begin{aligned}
%      \mathcal{P}_{expert} = M(\mathbf{p}_{persona}(x))
%  \end{aligned}
%  \label{eq:llm_generated_persona_selection}
%  \end{equation}

%  \noindent $\mathbf{p}_{persona}(x)$ indicates the system prompt that generates relevant for the given input $x$, which is inserted to LLM $M$ and generate relevant persona from it.

%  Since, handcrafted personas are generated based on the dataset explanation, they are not as specific as LLM-generated personas are in instance-by-instance basis.

% second draft - only using expert persona
In this section, We testified the performance between two different persona assigning methodologies via conducting a small experiment. The first method is using human handcrafted persona based on the dataset's explanation. Since every dataset has different explanation, each persona corresponding to dataset varies. Formally, if the question $x$ is from the dataset $d \in \mathcal{D}$, then handcrafted persona $\mathcal{P}_{d, fixed}$ is returned from function $f$ as follows:
\begin{equation}
\begin{aligned}
    \mathcal{P}_{d, fixed} = f(x, d) \:\:\:\:\: \\
    \textbf{where}\ d \in \{d'|d' \in \mathcal{D}\}
\end{aligned}
\label{eq:handcrafted_persona_selection}
\end{equation}
\noindent Where handcrafted Persona $\mathcal{P}_d$ is available when the given question $x$ is included in one of the datasets in $\mathcal{D}$.

The second method is leveraging persona generated by an LLM based on the given question. Inserting the question into the prompt, LLM infers an appropriate persona that could solve the given question. Suppose the given question is $x$, then the corresponding persona $\mathcal{P}_{expert}$ could be generated by the LLM as defined below:

 \begin{equation}
 \begin{aligned}
     \mathcal{P}_{expert} = M(\mathbf{p}_{persona}(x))
 \end{aligned}
 \label{eq:llm_generated_persona_selection}
 \end{equation}

 \noindent $\mathbf{p}_{persona}(x)$ indicates the system prompt that explains the LLM to generate a persona that is specialized to solve the given question $x$.

% 실험부분으로 빼기
Given two datasets, we annotate three different handcrafted persona for each dataset. In order to check the stability of each methodology, we compute the standard deviation which shows the variance of the performance of LLM. As shown in table \ref{table:variance_of_persona}, the standard deviation of using handcrafted persona is bigger than using LLM generated persona. The result presents that using LLM generated persona gives consistent results, providing confident evidence of the impact assigning persona to LLM. Thus, we designated using \textbf{LLM generated persona} as our method when utilizing persona assigned LLM.

\input{fig_texts/table:variance_of_persona}

\subsection{Generating personated and neutral perspective solutions}
 Once the persona is ready to use, the framework prepares two different settings of LLMs, one with persona, and the other without persona. Both LLMs are executed simultaneously, computing their own solution for the given input $x$. We follow the same implementation for the base model in \citet{kong2024better}. In formula, the following answers for each LLM is defined as the following:

 \begin{equation}
 \begin{aligned}
     S' = M(\mathbf{p}_{solve}(p, x)) \\
     S = M(x) \:\:\:\:\:\:\:\: \\
 \end{aligned}
 \label{eq:model_execution}
 \end{equation}

Where $p \in \{\mathcal{P}_{d, fixed}, \mathcal{P}_{expert}\}$ is the persona previously generated. Then both persona $p$ and the given input $x$ is inserted to a prompt $\mathbf{p}_{solve}$. After running through the LLM $M$ returns a solution $S'$. In case of using LLM without persona, the output $S$ is generated by inserting question directly into the LLM.
\subsection{Aggregating results of each LLM}
\label{eval LLM}
In this section, previously computed two solutions are introduced inside the LLM which is designated as an evaluator. Then the evaluator yields its decision indicated in 'A' or 'B'. The following mechanism is demonstrated in formula \ref{eq:evalLLM}.

\begin{equation}
\begin{aligned}
    C_{base, persona} = M_{\theta\{\tau,k\}}(\mathbf{p}_{eval}(x, S, S'))
\end{aligned}
\label{eq:evalLLM}
\end{equation}

The given input $x$, and two solutions ($S, S'$) generated from each LLMs is inserted into a evaluation prompt
$\mathbf{p}_{eval}$. Then the prompt is adapted into the LLM $M_{\theta}$ designated as an evaluator, which has the hyper-parameter $\theta$ indicating temperature $\tau$, and number of attempts $k$ which is going to be explained in section \ref{mitigate bias}. Eventually, $M_{\theta\{\tau,k\}}$ outputs a decision between two solutions into a symbol between 'A' and 'B'.

\subsection{Robust evaluation via mitigating bias}
\label{mitigate bias}

As introduced in Section \ref{eval LLM}, using the evaluator returns the final output of the framework;however this method contains position bias which hinders the total performance of the framework. In order to mitigate the following bias, we alternately insert both solutions into the evaluation prompt and execute the evaluator twice. Formally, given an input $x$, base output $S$, and output from the persona assigned LLM $S'$, we depict the process as the following:

\begin{equation}
\begin{aligned}
    C_{base, persona} = M_{\theta\{\tau,k\}}(\mathbf{p}_{eval}(x, S, S')) \\
    C_{persona, base} = M_{\theta\{\tau,k\}}(\mathbf{p}_{eval}(x, S', S)) \\
    t \gets t + 1 \:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\: \\
\end{aligned}
\label{eq:mitigation evaluation 1}
\end{equation}

By running the evaluator LLM twice via alternately inserting two solutions, the evaluator receives two decisions. Note that every time when two evaluators are executed for generating their decision, we count the number of attempt represented as $t$. Then the framework compares the two decision whether they are the same or not. Process reaches the end when these two decisions are same, otherwise the framework executes the process referred in equation \ref{eq:mitigation evaluation 1} again until their number of attempt $t$ is smaller than the model's max attempt decided as a hyper-parameter $k$. When $t$ gets bigger than $k$, then the process reaches the end returning the final output by giving $none$. The aforementioned process could be depicted as the following formula:

\begin{equation}
\resizebox{0.91\hsize}{!}{S_{final} &= 
    \begin{cases}
        S, & \textrm{if $C_{base,persona}=C_{persona,base}$ and $t < k$ } \\
        none & \textrm{if $t \geq k$}
    \end{cases}
}    
\end{equation}
